Understanding IoT Security Through the Data Crystal Ball: Where We Are Now and Where We Are Going to Be

Inspired by the boom of the consumer IoT market, many device manufacturers, start-up companies and technology giants have jumped into the space. Unfortunately, the exciting utility and rapid marketization of IoT, come at the expense of privacy and security. Industry reports and academic work have revealed many attacks on IoT systems, resulting in privacy leakage, property loss and large-scale availability problems. To mitigate such threats, a few solutions have been proposed. However, it is still less clear what are the impacts they can have on the IoT ecosystem. In this work, we aim to perform a comprehensive study on reported attacks and defenses in the realm of IoT aiming to find out what we know, where the current studies fall short and how to move forward. To this end, we first build a toolkit that searches through massive amount of online data using semantic analysis to identify over 3000 IoT-related articles. Further, by clustering such collected data using machine learning technologies, we are able to compare academic views with the findings from industry and other sources, in an attempt to understand the gaps between them, the trend of the IoT security risks and new problems that need further attention. We systemize this process, by proposing a taxonomy for the IoT ecosystem and organizing IoT security into five problem areas. We use this taxonomy as a beacon to assess each IoT work across a number of properties we define. Our assessment reveals that relevant security and privacy problems are far from solved. We discuss how each proposed solution can be applied to a problem area and highlight their strengths, assumptions and constraints. We stress the need for a security framework for IoT vendors and discuss the trend of shifting security liability to external or centralized entities. We also identify open research problems and provide suggestions towards a secure IoT ecosystem.

==> tables/imp_flaw_category.tex <==
\begin{table}[h]
\caption{Common Flaws in Implementation}
\label{tab:implementationflaw}
\scriptsize

\begin{center}
  \def\arraystretch{1.5}%  1 is the default, change whatever you need
  \setlength\tabcolsep{2pt} % default value: 6pt
\begin{threeparttable}
  \begin{tabular}{ c c c c c c c c}
  
  \toprule[0.12em]
  \shortstack{\textbf{Hardcode} \\ \textbf{credential}} & \shortstack{\textbf{Unencrypted} \\ \textbf{traffic}} & \shortstack{\textbf{Default} \\ \textbf{credentials}} & \shortstack{\textbf{XSS} \\ \textbf{CSRF}} & \shortstack{\textbf{Insecure} \\ \textbf{SSL}} & \shortstack{\textbf{Open} \\ \textbf{port}} & \shortstack{\textbf{Unverified} \\ \textbf{firmware}} & \textbf{Others} \\
  \hline
  
  12(19\%) & 9(14\%) & 4(6\%) & 3(5\%) & 3(5\%) & 2(3\%) & 2(3\%) & 27(43\%)\\
 
  
  \toprule[0.12em]
  

  \end{tabular}

\end{threeparttable}
\end{center}

\end{table}
